A Consistent Estimator for Confounding Strength

Regression on observational data can fail to capture a causal relationship in the presence of unobserved confounding. Confounding strength measures this mismatch, but estimating it requires itself additional assumptions. A common assumption is the independence of causal mechanisms, which relies on concentration phenomena in high dimensions. While high dimensions enable the estimation of confounding strength, they also necessitate adapted estimators. In this paper, we derive the asymptotic behavior of the confounding strength estimator by Janzing and Sch\"olkopf (2018) and show that it is generally not consistent. We then use tools from random matrix theory to derive an adapted, consistent estimator.

==> chapters/Experiments.tex <==
\section{Experiments}\label{sec:experiments}

\textbf{Baselines.} We empirically evaluate the performance of the RMT-estimator ($\confRMT$) against three different baselines. A first and natural baseline to compare against is the plugin estimator ($\confPlugin$) \citep{Jan:2018}. Recall that the plugin estimator for confounding strength is specified by the two quantities $\tauPlugin$ and $\thetaPlugin$. 
% While both $\tauPlugin$ and $\thetaPlugin$ are biased estimators of $\tauPop$ and $\thetaTrue$, unlike for $\thetaPlugin$, where estimating its bias is as hard as estimating $\thetaTrue$ itself, the bias of $\tauPlugin$ can be easily estimated from observed quantities $n, d$. 
While both $\tauPlugin$ and $\thetaPlugin$ are biased estimators of $\tauPop$ and $\thetaTrue$, the bias of $\tauPlugin$ can be easily estimated from observed quantities $n, d$, whereas estimating the bias of $\thetaPlugin$ is as hard as estimating $\thetaTrue$ itself.
To elicit the influence of a biased estimation of $\thetaTrue$, we additionally consider a \textit{$\tau$-corrected} estimator of confounding strength as our second baseline. Formally, we define $\confTcorr \coloneqq 1 - 1/(1 + \tauRMT \cdot \thetaPlugin)$, that is, we simply replace the $\tauPlugin$ of the plugin estimator by the RMT-corrected $\tauRMT$. The third baseline we consider is what we refer to as the \textit{population} estimator ($\confPop$) which estimates confounding strength assuming the full knowledge of the \textit{observational} distribution. Note that this is distinct from the \textit{ground truth} confounding strength $\confTrue$, which requires the full knowledge of the \textit{interventional} distribution.  

\begin{figure}
    \includegraphics[width=0.8\textwidth]{journal_paper/fig/conf/conf_d_gamma_grid.pdf}\hfill
    \caption{Behavior of the 4 estimators: $\confPop$, $\confPlugin$, $\confRMT$, and $\confTcorr$ for different $(d, \gamma)$ settings under the data generation process described in Section \ref{sec:experiments}. We chose the parameters $\tilde{\gamma} = l / d = 1.2$ and $c = 1/ 3$. The figure clearly shows that while the plugin estimators are biased, the RMT estimator consistently estimates the true confounding strength.}
    \label{fig:conf_d_gamma}
\end{figure}
 
\noindent\textbf{Data generation.} To specify our distribution of causal models, for some $d \in \R$, we first draw eigenvalues values $\mycurls{\lambda_i}_{i=1}^d$ according to a \textit{Marchenko Pastur law} \citep{Bai:2010} which, for some $c \in (0, 1)$, is defined as 
 \begin{equation}
     \label{eq:mp_law}
     \mu(d\lambda) = \frac{1}{2 \pi c \lambda} \sqrt{(\lambda - c_{-})^+ (c_{+} - \lambda)^+} d\lambda,
 \end{equation}
 where $c_{\pm} = (1 \pm \sqrt{c})^2$ and $(z)^+ = \max(0, z)$. For some $l > d$, we specify the mixing matrix $M \in \R^{d \times l}$ according to its singular value decomposition as $U \Lambda V^T$, where $\Lambda \in \R^{d \times l}$ is a rectangular diagonal matrix with singular values $\mycurls{\sqrt{\lambda_i}}_{i=1}^d$ on the diagonal and $U, V$ are random orthogonal matrices in $\R^{d \times d}$ and $\R^{l \times l}$ respectively. This generating procedure for $M$ can be viewed as a generalization of independently and randomly drawing entries of $M \in \R^{d \times l}$ according to a standard normal distribution since under this generation, the spectrum of $\Sigma = MM^T$ asymptotically follows a Marchenko Pastur Law with $c = d / l$. Generating the singular values of $M$ for some arbitrary $c < 1$ (independently of $d, l$), therefore allows us to consider a broader range of models. 
 
 We then generate parameters $\sigma_{\alpha}$ and $\sigma_{\beta}$ such that the confounding strength is asymptotically uniformly distributed between $0$ and $1$. Specifically, we generate parameters $\zeta', \sigma_{\beta}$ uniformly in $[0, 1]$ and $[0, 3]$ respectively and we define $\sigma_{\alpha}$ as $ (\sigma_{\beta}\cdot(1 - \zeta') + \zeta' \cdot \tauPop)/(1 - \zeta')$. Given a mixing matrix $M$ and parameters $\sigma_{\alpha}, \sigma_{\beta}$, to generate a causal model, we draw $\alpha$ and $\beta$ according to normal distributions $\mathcal{N}(0, \sigma_{\alpha} I_{l})$ and $\mathcal{N}(0, \sigma_{\beta} I_{d})$ respectively. Samples from the observational distribution are then drawn according to the structural equations specified in \eqref{eq:causal_model}.
 
\noindent\textbf{Results: influence of $d,\gamma$ on the estimation of $\confTrue$.} To understand the influence of the covariate dimension $d$ and overparameterization ratio $\gamma$, we compare the different estimators against the ground truth by varying $d$ and $\gamma$ while fixing the dimension of the hidden confounders as $l = a \cdot d$ for some $a > 1$. Figure \ref{fig:conf_d_gamma} shows the results from this experiment. As expected, it shows that for a fixed $\gamma$, all the estimators increasingly concentrate in higher dimensions. In smaller dimensions, it also shows that the population estimator can considerably deviate from the ground truth reflecting the underlying non-identifiability issue at finite $d$. For a fixed $d$, the hardness of the problem increases with $\gamma$ for all the estimators except $\confPop$ which is of course independent of $\gamma$. We also see in this plot that all the estimators including $\confPlugin$ and $\confTcorr$ closely track the ground truth for larger $d$ and as $\gamma$ close to $0$. This is in line with what the theory suggests since $\thetaPlugin$ consistently estimates $\thetaTrue$ as $\gamma \rightarrow 0$. Finally, we see that while the RMT estimator remains close to the ground truth with increasing $\gamma$, both $\confPlugin$ and $\confTcorr$ are systematically biased. While $\confPlugin$ significantly overestimates the confounding strength as $\gamma$ approaches $1$ due to a large overestimation of $\tauPop$, $\confTcorr$ systematically underestimates $\confTrue$ since, as we will see later, $\thetaTrue$ is underestimated. Note that this behavior depends on the ratio $\Tilde{\gamma} = l/d$ and cannot be generalized to all experimental settings. The bias of $\thetaPlugin$ has a highly complex dependence on $\tilde{\gamma}$ and as mentioned in Section \ref{sec:population_and_plugin}, estimating $\tilde{\gamma}$ is as hard as estimating $\zeta$ itself. The RMT estimator $\confRMT$, on the other hand, remains consistent independently of $\tilde{\gamma}.$

% We will discuss this further in our discussion of the dependence of various estimators on $\Tilde{\gamma}.$
 

% \noindent\textbf{Influence of $\Tilde{\gamma}$.}

% \TODO{Don't talk about gammatilde in the first version.}

% \subsection{Estimation of $\theta^*$.}
% \leena{We may want to talk about other quantities such as log quadform.}





